Query the model: precomputations for efficient inference with Bayesian Networks

Variable Elimination is a fundamental algorithm for probabilistic inference over Bayesian networks. In this paper, we propose a novel materialization method for Variable Elimination, which can lead to significant efficiency gains when answering inference queries. We evaluate our technique using real-world Bayesian networks. Our results show that a modest amount of materialization can lead to significant improvements in the running time of queries. Furthermore, in comparison with junction tree methods that also rely on materialization, our approach achieves comparable efficiency during inference using significantly lighter materialization.

==> extensions_original.tex <==
\section{Extensions}
\label{sec:extensions}

\subsection{Space budget constraints}
\label{sec:space-budget}

The algorithms we presented in the previous section 
address Problem~\ref{problem:qtm}, 
where a budget \budget is given on the number of nodes to be materialized. 
A more realistic and practical scenario is Problem~\ref{problem:qtm-space}, 
where a budget \spacebudget is given on the total space required to materialize the selected nodes. 
In this case, for each node \nodeu of the elimination tree \tree
the space~$\weight{\nodeu}$ required to materialize the probability table at node \nodeu
is specified as input. 

Both of the algorithms we presented in the previous section, 
dynamic-programming and greedy, 
can be extended to address this more general version of the problem.
In both cases the extension is fairly standard, 
and for lack of space we only describe it here in brief.

For the dynamic-programming algorithm the idea is to create an entry
\DPtable{\nodeu}{\partialbudget}{\nodev}
for nodes \nodeu and \nodev, 
and index \partialbudget taking values from 1 to $\min\{\spacebudget,\totalweight{\nodeu}\}$, 
where \totalweight{\nodeu} is the total space required to materialize 
the probability tables of all nodes in~\subtree{\nodeu}.
We then evaluate the entry 
\DPtable{\nodeu}{\partialbudget}{\nodev}
by considering the maximum benefit over all possible values 
\partialbudgetl and \partialbudgetr such that 
$\partialbudgetl+\partialbudgetr = \partialbudget-\weight{\nodeu}$, 
where \weight{\nodeu} is the space required to materialize node \nodeu.

The modified algorithm provides the exact solution, 
and the running time is $\bigO{\nonodes\height\spacebudget^2}$.
Note, however, that unlike the previous case (Problem~\ref{problem:qtm}) 
where \budget is bounded by \nonodes, 
the value of \spacebudget is not bounded by \nonodes. 
As the running time is polynomial in the \emph{value} of \spacebudget, 
which can be specified by $\bigO{\log\spacebudget}$ bits, 
it follows that the algorithm is in fact \emph{pseudo-polynomial}.
However, the technique can be used to obtain
a fully-polynomial approximation scheme (FPTAS)
by rounding all space values into a set of smaller granularity 
and executing the dynamic programming algorithm using these rounded values. 

For the greedy algorithm, 
in each iterative step
we select to materialize the node \nodeu that maximizes the 
\emph{normalized marginal gain}
$\left(\benefit{\solution \cup \{\nodeu\}} - \benefit{\solution}\right)/\weight{\nodeu}$.
The modified greedy algorithm has the same running time
and yields the same approximation guarantee
$\left(1-\frac 1e\right)$.

\subsection{Accounting for redundant variables}
\label{sec:redundant}

In our algorithms so far we have considered 
a \emph{fixed} elimination tree \tree and elimination order \eliminationOrder.
The elimination~tree \tree specifies 
% the computations that are performed for the evaluation of a query \query\ 
% --- essentially, 
the order in which sums-of-products evaluations are performed, 
with one summation for \emph{every variable} in~\bayesianNet.
% as described in Section~\ref{sec:setting}.
One can observe, however,  that 
it is \emph{not} necessary to involve \emph{every variable} in the evaluation of a query.
For example, for the Bayesian network \bayesianNet shown in Figure~\ref{fig:redundant}, 
the query $\query_1 = \prob{\varb = \varbvalue, \varc}$
can be computed from the sub-network $\bayesianNet_1 \subseteq \bayesianNet$, 
while the query $\query_2 = \prob{\varc \mid \varb = \varbvalue}$
can be computed from the sub-network $\bayesianNet_2 \subseteq \bayesianNet$.



\begin{figure}
\begin{tabular}{c||c|c|c|c}
$\mathcal N$ & $\mathcal N_1$ &  $\mathcal N_2$ &$\mathcal N_3$ & $\mathcal N_4$\\ %\hline
\includegraphics[width=0.14\columnwidth]{img/redundant0.png} &
\includegraphics[width=0.14\columnwidth]{img/redundant1.png} &
\includegraphics[width=0.14\columnwidth]{img/redundant2.png} &
\includegraphics[width=0.14\columnwidth]{img/redundant3.png} &
\includegraphics[width=0.14\columnwidth]{img/redundant4.png} % \\ \hline
\end{tabular}
\caption{The input Bayesian network \bayesianNet and some of its sub-networks. Some variables in \bayesianNet may be redundant for the evaluation of some queries, allowing us to perform computations over ``shrunk'' networks.}
\label{fig:redundant}
\end{figure}

Previous work~\cite{geiger1990d,lauritzen1988local,zhang1994simple}
provides methods to determine the variables that are \emph{redundant} for the evaluation of a query \query\  
allowing us to perform computations based on a ``shrunk'' Bayesian network.
% i.e., the sub-network induced from \bayesianNet by the non-redundant variables.
The characterization of variables into redundant and non-redundant is given in Theorem~\ref{thm:redundant}, 
based on the following two definitions.
\begin{definition}[Moral graph~\cite{zhang1994simple}] 
The moral graph \moralGraph of a Bayesian network \bayesianNet 
is the undirected graph that results from \bayesianNet 
after dropping edge directions and 
adding one edge for all pairs of nodes that share a common child. % in~\bayesianNet.
\end{definition} 
\begin{definition}[\separated variables~\cite{zhang1994simple}] 
Two\\vari\-ables \vara and \varb in a Bayesian network \bayesianNet
are said to be \separated by variables \somevars 
if removing \somevars from the moral graph \moralGraph of \bayesianNet leaves no 
(undirected) path between \vara and \varb in \moralGraph. 
This property is denoted as \isseparated{\vara}{\varb}{\somevars}.
\end{definition}
\begin{theorem}[Redundant Variables~\cite{zhang1994simple}]
Let \bayesianNet be~a Bayesian network  and 
$\query = \prob{\qvarfree, \qvarbound=\qvarvals \mid \qvarbound'=\qvarvals'}$ a query. 
Let \ancestors{} be the union of ancestors in \bayesianNet of all variables in \query:
\[
\ancestors{} = \cup_{x\in\qvarfree\cup\qvarbound\cup\qvarbound'}\ancestors{x}.
\]
Also, let 
\redundantmarginal be all variables outside \ancestors{}, 
i.e., $\redundantmarginal = \allvars \setminus \ancestors{}$,
and \redundantconditional all ancestor nodes \ancestors{} that are 
\separated from $\qvarfree\cup\qvarbound$ by $\qvarbound'$, i.e., 
\[
\redundantconditional = \{\vara\in\ancestors{} \mid \isseparated{\vara}{\varb}{\qvarbound'} \text{ for all } \varb\in\qvarfree\cup\qvarbound\}.
\]
The variables in $\redundantvars = \redundantmarginal\cup\redundantconditional$ are redundant, 
and no other variables are redundant.
\label{thm:redundant}
\end{theorem}
Given a Bayesian network \bayesianNet and a query \query
we write $\shrink{\query, \bayesianNet}$ 
(or $\shrink{\query}$ when \bayesianNet is understood from the context)
to denote the Bayesian network 
that results from the removal of all redundant variables as per Theorem~\ref{thm:redundant}.
We can evaluate the query \query on a shrunk Bayesian network \resultBN, 
such that $\shrink{\query} \subseteq \resultBN \subseteq \bayesianNet$,
by building an elimination tree $\tree'$ on \resultBN 
and obtain immediate efficiency gains.
However, the elimination tree $\tree'$ that is built on $\resultBN$ 
codifies different computations than the tree \tree built on \bayesianNet, 
even if $\tree'\subseteq\tree$.
Therefore, the tables of factors we materialize for \tree 
using the algorithms of Section~\ref{sec:algorithms} 
do not generally correspond to factor tables for $\tree'$.
In the next section we discuss how to address
the issue of evaluating different queries while accounting for redundant variables.

\subsubsection{Redundancy-aware scheme}
\label{sec:scheme}

The main idea of our \emph{redundancy-aware scheme} 
is to materialize different probability tables for a set of ``shrunk'' Bayesian networks 
obtained through removal of redundant variables.
% We start by describing the basic components of the scheme,
% and then discuss how each component is built and how it operates.
The scheme consists of the following components:

\begin{figure}
\begin{center}
\includegraphics[width=0.3\columnwidth]{img/lattice.png}
\end{center}
\caption{Instance of a lattice of Bayesian networks, for the networks that appear in Figure~\ref{fig:redundant}.}
\label{fig:lattice}
\end{figure}


\spara{Lattice of Bayesian networks}. Consider a set of Bayesian networks 
$\lattice = \{\bayesianNet_0, \bayesianNet_1, \bayesianNet_2, \ldots, \bayesianNet_\latticeSize\}$ that includes the input Bayesian network $\bayesianNet = \bayesianNet_0$ and $\latticeSize$ of its subnetworks, 
each of which is induced by a subset of variables:
\[
\bayesianNet_0 = \bayesianNet;\; \bayesianNet_i \subseteq \bayesianNet, \text{ for all } i = 1,\ldots,\latticeSize.
\]
The set \lattice can be represented as a lattice where edges are added
between each network and its maximal subnetworks in \lattice 
(see an example in Figure~\ref{fig:lattice}).

\spara{Query-network mapping}. 
Consider a function $\mapping: \queriesset\rightarrow \lattice$
(where \queriesset is the set of all possible queries)
that maps a query $\query\in\queriesset$ to a Bayesian network $\bayesianNet_i\in\lattice$
from which the answer to \query can be computed exactly. 
Notice that there is always such a Bayesian network in the lattice, namely the input Bayesian network $\bayesianNet_0 = \bayesianNet$.

\spara{Query workloads}. 
Each Bayesian network $\bayesianNet_i\in\lattice$ 
is associated with a query workload, characterized by: 
($i$) the probability $\bnProb_i$ that a random query is mapped to $\bayesianNet_i$;
%  with $\pi_i\geq 0$ and $\sum_{i=0}^\latticeSize{ \bnProb_i } = 1$; 
($ii$) a probability distribution $\netprob{i}{\query} = \prob{\query \mid \bayesianNet_i}$ 
over the queries that are mapped to~$\bayesianNet_i$.

\smallskip
We now discuss how the scheme operates and how its components are built.
When a query arrives it is mapped to one network in the lattice 
from which its value is computed exactly. 
As we discuss below, this mapping operation can be performed efficiently. 
In this scheme, offline optimization considerations include 
the choice of networks to include in the lattice, 
as well as the materialization of factors for each network. 
We discuss them below.

\spara{An algorithm for query-network mapping.}
Algorithm~\ref{algo:map} finds the smallest % (in terms of node-size) 
Bayesian network \resultBN 
in the lattice such that $\shrink{\query} \subseteq \resultBN \subseteq \bayesianNet$
that can be used to answer a query \query. 
The algorithm proceeds as follows: 
first, at line~\ref{line:shrink}, it computes the smallest 
% (in terms of node-size) 
shrunk network \shrunkBayesianNet = \shrink{\query} 
that can be used to answer query \query exactly; 
% (this can be done in time $\bigO{|\edges|}$ as per Theorem~\ref{thm:redundant}); 
then, it performs a breadth-first-search on the lattice \lattice 
starting from the top element % (input Bayesian network \bayesianNet) 
but does not extend search paths on which it encounters networks \otherBayesianNet 
that do not include $\shrunkBayesianNet$ as subnetwork.
% (line~\ref{line:subnetworkTest}). 

To test whether $\shrunkBayesianNet\subseteq\otherBayesianNet$, it is sufficient to test whether the intersection of the (labeled) edge-sets of the two networks is not empty,
which can be done in time $\bigO{|\edges|\log(|\edges|)}$.
% Notice also (line~\ref{line:noDuplicates}) that the algorithm does not visit twice the same Bayesian network in the lattice, as it requires each tested Bayesian network to be strictly smaller than the best found up to that point.
The algorithm finds the correct network in the lattice since, by construction, 
if it has visited a Bayesian network \otherBayesianNet that contains the target \resultBN as subnetwork, 
there is a path from \otherBayesianNet to \resultBN, 
and this condition holds for the best (smallest Bayesian network that contains \shrunkBayesianNet) 
discovered up to any point during the execution of the algorithm.
The total running time in terms of subnetwork tests
%  (evaluations of $\shrunkBayesianNet\subseteq\otherBayesianNet$ in line~\ref{line:subnetworkTest}) 
is $\bigO{\latticeSize\,|\edges|\log(|\edges|)}$.

\begin{algorithm}[t]
\begin{small}
\begin{algorithmic}[1]
\caption{\label{algo:map}Map(\lattice, \query)}
\State Let $\shrunkBayesianNet \assign \shrink{\query}$\label{line:shrink}
\State Let $\queue \assign [\bayesianNet]$
\State Let $\resultBN \assign \bayesianNet$
\While{$\queue\not = \emptyset$}
	\State \otherBayesianNet = \deque{\queue}
	\If{$\|\otherBayesianNet\|<\resultBN$ \label{line:noDuplicates} }
		\If{$\shrunkBayesianNet\subseteq\otherBayesianNet$ \label{line:subnetworkTest} }
			\State $\resultBN\assign\otherBayesianNet$
			\For{$\yetAnotherBayesianNet\in\children{\otherBayesianNet}$}
				\State \enque{\yetAnotherBayesianNet, \queue}
			\EndFor
		\EndIf
	\EndIf
\EndWhile
\State \Return \resultBN
\end{algorithmic}
\caption{\label{algo:map}Map(\lattice, \query)}
\end{small}
\end{algorithm}


\mpara{Building the lattice.} 
We build the lattice \lattice off-line, in three phases.
During the first phase, we consider the full lattice \fullLattice that includes all sub-networks of \bayesianNet\ 
and estimate the probability $\fullBNProb_i$ that a random query \query has 
$\bayesianNet_i = \shrink{\query} \in\fullLattice$ as its corresponding ``shrunk'' network. 
Notice that, for the full lattice, $\fullBNProb_i$ is also the probability that a random query is mapped by Algorithm~\ref{algo:map} to Bayesian network $\bayesianNet_i\in\fullLattice$.
In practice, we consider a sample of queries \query 
(either from a query-log or a probabilistic model) and estimate $\fullBNProb_i$ 
as the relative frequency with which network $\bayesianNet_i$ is the ``shrunk'' network 
that can be used to evaluate \query.

During the second phase, we choose a small number \latticeSize of networks from \fullLattice 
% (other than the input Bayesian network) 
to form lattice \lattice. 
We want to build a lattice of networks that captures well the distribution \fullBNProb.
%  --- for example, to choose the \latticeSize networks with highest \fullBNProb. 
%% Another approach is to consider some notion of \emph{utility} for the $\latticeSize$ chosen networks that form lattice \lattice: a chosen lattice will have higher utility if it allows us to evaluate a workload of queries more efficiently compared to evaluating all queries directly from the input network \bayesianNet. 
In practice, we use a greedy approach, 
successively choosing to add to \lattice the network that optimizes the utility of the lattice. 
% Such an approach is used by \cite{harinarayan1996datacubes} to build a lattice for the efficient computation of data cubes.
% 
During the third phase, % having already built a lattice \lattice, 
we follow an approach similar to the first phase to estimate anew the probability $\bnProb_i$ 
that a random query \query has $\bayesianNet_i = \shrink{\query} \in\lattice$ 
as its corresponding ``shrunk'' Bayesian network, 
as well as the probability distribution $\netprob{i}{\query} = \prob{\query \mid \bayesianNet_i}$ 
over the queries \query that are mapped to $\bayesianNet_i$.

\mpara{Optimal materialization.} 
Given the set \lattice of networks contained in the lattice, 
a query workload $(\bnProb_i, \netprob{i}{\query})$ over the networks, and a budget $\budget$, 
we wish to materialize $\budget_i$ factors for Bayesian network $\bayesianNet_i$, 
with $\sum_{i=0}^{\latticeSize}\budget_i\leq\budget$,
so that
$\globalbenefit{\{\budget_i\}}=\sum_{i=0}^{\latticeSize}\bnProb_i \optimalbenefit{i}{\budget_i}$ is maximized, 
where $\optimalbenefit{i}{\budget_i}$ is the optimal benefit obtained by solving problem~\ref{problem:qtm} for Bayesian network $\bayesianNet_i$ with budget $\budget_i$.
Let \globallyoptimalbenefit{m, \budget} be the optimal value of 
% \globalbenefit{\{\budget_i;\ \text{s.t.}\ \budget_i = 0\ \text{for}\ i = (m+1)..\latticeSize\}} 
\globalbenefit{\cdot}
for the first $m$ networks of \lattice, with budget \budget. Then the following equation holds
\[
\globallyoptimalbenefit{m+1, \budget} = \max_\partialbudget\{\bnProb_{m+1}\optimalbenefit{i}{\partialbudget} + \globallyoptimalbenefit{m, \budget - \partialbudget}\}\,,
\]
and defines a dynamic-programming algorithm to compute the optimal materialization over a set of networks \lattice.
% 	\item This can be done optimally with a DP programming.
% 	\item DP formula for optimal benefit: 
% \[
% 	OPT[i;k] = \max_\kappa\{\pi_i opt[i;\kappa] + OPT[i+1; k - \kappa]\}
% \]

